MultiON: Benchmarking Semantic Map Memory using Multi-Object Navigation

Navigation tasks in photorealistic 3D environments are challenging because they require perception and effective planning under partial observability. Recent work shows that map-like memory is useful for long-horizon navigation tasks. However, a focused investigation of the impact of maps on navigation tasks of varying complexity has not yet been performed. We propose the multiON task, which requires navigation to an episode-specific sequence of objects in a realistic environment. MultiON generalizes the ObjectGoal navigation task and explicitly tests the ability of navigation agents to locate previously observed goal objects. We perform a set of multiON experiments to examine how a variety of agent models perform across a spectrum of navigation task complexities. Our experiments show that: i) navigation performance degrades dramatically with escalating task complexity; ii) a simple semantic map agent performs surprisingly well relative to more complex neural image feature map agents; and iii) even oracle map agents achieve relatively low performance, indicating the potential for future work in training embodied navigation agents using maps. Video summary: https://youtu.be/yqTlHNIcgnY

==> notes.tex <==






















\begin{table}
\ra{1.3}
\centering
\caption{\todo{Caption. Baselines(Max Steps: 2500)}}
\label{tab:random-baselines-overall-metrics}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}l rrr rrr rrr rrr @{}}
\toprule
 & \multicolumn{3}{c}{Percentage Success} & \multicolumn{3}{c}{Success} & \multicolumn{3}{c}{MO-SPL} & \multicolumn{3}{c}{PS-SPL}\\ \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
 & \mon{1} & \mon{2} & \mon{3} & \mon{1} & \mon{2} & \mon{3} & \mon{1} & \mon{2} & \mon{3} & \mon{1} & \mon{2} & \mon{3}\\
\midrule
\texttt{Random} & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$\\
\texttt{Random + Oracle Found} & $0.26$ & $0.16$ & $0.12$ & $0.26$ & $0.08$ & $0.024$ & $0.08$ & $0.02$ & $0.01$ & $0.08$ & $0.05$ & $0.04$\\
\texttt{Forward + Oracle Found} & $0.013$ & $0.007$ & $0.005$ & $0.013$ & $0$ & $0$ & $0.012$ & $0$ & $0$ & $0.012$ & $0.07$ & $0.005$\\
\bottomrule
\end{tabular}
}
\end{table}


\begin{table}
\ra{1.3}
\centering
\caption{\todo{Caption. Baseline(Max Steps: 500)}}
\label{tab:random-baselines-overall-metrics-500}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}l rrr rrr rrr rrr @{}}
\toprule
 & \multicolumn{3}{c}{Percentage Success} & \multicolumn{3}{c}{Success} & \multicolumn{3}{c}{MO-SPL} & \multicolumn{3}{c}{PS-SPL}\\ \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
 & \mon{1} & \mon{2} & \mon{3} & \mon{1} & \mon{2} & \mon{3} & \mon{1} & \mon{2} & \mon{3} & \mon{1} & \mon{2} & \mon{3}\\
\midrule
\texttt{Random} & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$ & $0$\\
\texttt{Random + Oracle Found} & $0.09$ & $0.05$ & $0.03$ & $0.09$ & $0.02$ & $0.005$ & $0.02$ & $0.008$ & $0$ & $0.02$ & $0.013$ & $0.009$\\
\texttt{Forward + Oracle Found} & $0.004$ & $0.001$ & $0$ & $0.004$ & $0$ & $0$ & $0.001$ & $0$ & $0$ & $0.001$ & $0$ & $0$\\
\bottomrule
\end{tabular}
}
\end{table}

==> sections/additional.tex <==
\section{Additional Material}

\SW{
\subsection{Visualizing learnt models through Grad-CAM}
To understand what parts what parts of the map or the RGBD frame the model is attending to while choosing an action, we visualize the gradient-weighted Class Activation Maps (Grad-CAM)~\cite{selvaraju2016grad} of the two. For doing so, we use the gradients of the sampled action (likely to be the action with a higher score) flowing into the final constitutional layer. We do this for both the CNNs: the one  processing the Map and the one processing the RGBD frame and produce a localization map highlighting the important regions in the map for the predicted action. 

\textit{There doesn't seem to be anything interesting in the visualizations, what frame should I put here? The only time something slightly remarkable appears in the visualizations is when an object is in view and the heatmap is focused on it.}
}

